Precise Attack Synthesis for Smart Contracts

Smart contracts are programs running on top of blockchain platforms. They interact with each other through well-defined interfaces to perform financial transactions in a distributed system with no trusted third parties. But these interfaces also provide a favorable setting for attackers, who can exploit security vulnerabilities in smart contracts to achieve financial gain. This paper presents SmartScopy, a system for automatic synthesis of adversarial contracts that identify and exploit vulnerabilities in a victim smart contract. Our tool explores the space of \emph{attack programs} based on the Application Binary Interface (ABI) specification of a victim smart contract in the Ethereum ecosystem. To make the synthesis tractable, we introduce \emph{summary-based symbolic evaluation}, which significantly reduces the number of instructions that our synthesizer needs to evaluate symbolically, without compromising the precision of the vulnerability query. Building on the summary-based symbolic evaluation, SmartScopy further introduces a novel approach for partitioning the synthesis search space for parallel exploration, as well as a lightweight deduction technique that can prune infeasible candidates earlier. We encoded common vulnerabilities of smart contracts in our query language, and evaluated SmartScopy on the entire data set from etherscan with $>$25K smart contracts. Our experiments demonstrate the benefits of summary-based symbolic evaluation and show that SmartScopy outperforms two state-of-the-art smart contracts analyzers, Oyente and Contractfuzz, in terms of running time, precision, and soundness. Furthermore, running on recent popular smart contracts, SmartScopy uncovers 20 vulnerable smart contracts that contain the recent BatchOverflow vulnerability and cannot be precisely detected by existing tools.

==> algorithm.tex <==
\section{Algorithm}\label{sec:algo}
In this section, we introduce the high-level idea of our synthesis algorithm, 
leaving the discussion of symbolic evaluation and vulnerability queries
 to section~\ref{sec:exe} and section~\ref{sec:query}, respectively.

Algorithm~\ref{alg:synthesis} describes the pseudocode of our top-level 
synthesis algorithm. In particular, given an initial state $\pstate$, 
a query $\query$ for a security property, and all publicly available 
components $\comps$ of a given contract, the {\sc Synthesize} procedure 
either returns an attack program that satisfies $\query$ or produces 
$\bot$, meaning that no such program exists.

Specifically, the {\sc Synthesize} routine maintains a priority queue 
$\worklist$ of all available sketches. At the beginning, our $\worklist$
only contains $\sketch_0$, representing a set of all possible programs.
In each iteration of the main loop (line 5-14), the algorithm picks a
sketch $\sketch$ from $\worklist$ and uses the {\sc instantiation} rule
in Figure~\ref{fig:sketch} to figure out a set of instantiations using 
components from $\comps$ (line 8). 

Then for each instantiation $\sketch_i$, we symbolically evaluate (line 9, 
will further elaborate it in section~\ref{sec:exe}) it on the initial 
state $\pstate$, and the evaluation will return $\pstate^{*}$ as all reachable
states starting from $\pstate$. 

Now, given a query $\query$ regarding a specific security property (e.g., out-of-gas, overflow, etc), 
at line 10, we invoke the built-in function {\sc solve} from our underlying engine~\cite{rosette}, and 
the {\sc solve} function essentially encodes all reachable states in $\pstate^{*}$ as an 
SMT formula and asks whether there exists a model (i.e., a reachable state) such that 
$\query$ holds. If the answer is {\sc true}, then it will return a model $I_b$ which maps 
holes (i.e., symbolic values) to concrete values. Consequently, the {\sc bind} routine will accept $I_b$ and sketch $\sketch_i$ as input, and return a concrete attack program $p$ (line 12).  

On the other hand, if the answer at line 10 is {\sc false}, our algorithm performs 
sketch refinement at line 14. The intuition behind our sketch refinement is to apply
the {\sc expansion} rule in Figure~\ref{fig:sketch} 
on current sketch $\sketch$ to obtain sketches of longer size, which will 
be added to the priority queue $\worklist$ for future iterations.
\begin{algorithm}[t]
\caption{Synthesis Algorithm}\label{alg:synthesis}
{%\small 
\begin{algorithmic}[1]
%\vspace{0.05in}
\Procedure{Synthesize}{$\pstate, $\query$, \comps$}
%\vspace{0.05in}
\State {\rm \bf input:} Initial state $\pstate$, query $\query$,  and components $\comps$

%\State \ \ \ \ \ \ \ \ \ \ \ \ components $\comps$, and tests $\tests$
\State {\rm \bf output:} Synthesized program or $\bot$ if failure
\vspace{0.05in}

\State  $\worklist :=$  \{$\sketch_0$\} \Comment{ \ Init worklist}

\While {$\worklist \neq \emptyset$} 
    \State {\rm choose} $\sketch \in \worklist$;     
    \State $\worklist := \worklist \backslash \{\sketch\}$ \Comment{Pick a component}
        \For{$\sketch_i \in$ {\sc instantiate}($\sketch)$}
            \State $\pstate^{*}$ := $\peval{\sketch_i}$ \Comment{Symbolic evaluation}
            \State $I_{b}$ := {\sc solve}($\pstate^{*}, \query$) 
            %\State \Comment{Sketch completion}
            \If{{\sc SAT}=$I_{b}$}
            	\State $p$ := {\sc bind}($I_{b}, \sketch_i$) \Comment{Fill $\sketch_i$ with $I_b$}
                \State \Return $p$
            \EndIf
        \EndFor
    \State $\worklist$ := $\worklist \cup$ {\sc refine}($\sketch$) \Comment{Sketch refinement}
\EndWhile
\vspace{0.05in}
\State \Return $\bot$
\EndProcedure
\end{algorithmic}
}
\end{algorithm}
\paragraph{Discussion.}
The {\sc Synthesize} routine is sound, and it is complete modulo sketches of 
size up to a certain $K$. That is, if the shape of an attack program $p$ 
belongs to one of the sketches in our priority queue $\worklist$, 
then Algorithm~\ref{alg:synthesis} will return a solution.
Based on the above discussion, we can state the following theorems. 
\begin{theorem}{{(\bf Soundness)}}
If {\sc Synthesize} returns an attack program $p$, and we reach a new program state $\pstate$
by executing $p$, then query $\query$ holds on $\pstate$.
\end{theorem}
\begin{theorem}{{(\bf Completeness)}}
If executing an attack program $p$ reaches a program state on which $\query$ holds,
and program $p$ belongs to one of the sketches in our priority queue,
then {\sc Synthesize} will eventually generate such an attack program. 
\end{theorem}

